Atomic Parity-Violation and Precision Physics

The atomic parity-violation (APV) parameter QW for a nucleus with `n' neutrons and `z' protons has been included in the list of pseudo-observables accessible with the codes TOPAZ0 and ZFITTER. In this way one can add the APV results in the LEP EWWG `global' electroweak fits, checking the corresponding effect when added to the existing precision measurements.

==> Lessons_def.tex <==
\newcommand{\mtl}{ m_t }
\newcommand{\mzl}{ M_{\sss Z}}
\newcommand{\mzf}{ M_{\sss Z}^4 }
\newcommand{\lpstnt}{ {\hat L}_0(\mtl,0,\mtl)    }
\newcommand{\lpstzn}{ {\hat L}_0(\mtl,\mzl,0)    }
\newcommand{\lpstzs}{ {\hat L}_0(\mtl,\mzl,0)    }
\newcommand{\lpttzt}{ {\hat L}_0(\mtl,\mzl,\mtl) }
\newcommand{\plstnt}{ {\hat L}_1(\mtl,0,\mtl)    }
\newcommand{\plstzn}{ {\hat L}_1(\mtl,\mzl,0)    }
\newcommand{\plstzt}{ {\hat L}_1(\mtl,\mzl,\mtl) }
\newcommand{\plttzt}{ {\hat L}_1(\mtl,\mzl,\mtl) }

\newcommand{\Lnmuzm}{L_{\tHs}(\mzl)}
\newcommand{\Lnmutm}{L_{\tHs}(\mtl)}

\newcommand{\vts}{v^2_t}
\newcommand{\vt }{v_t}
\newcommand{\at }{a_t}
\newcommand{\ats}{a^2_t}

\newcommand{\DGrt  }{\Delta}
 
\newcommand{\nll }{\nonumber \\}
\newcommand{\Simplexl }{\int_0^1 dx }
\newcommand{\Simplexll}{\int_0^1 dx \int_0^{1-x} dy}
\newcommand{\Poly}[1]{P_{x,y}^{#1}}
\newcommand{\DettI}{\ds \frac{1}{\Delta}}

\newcommand{\xvarl}{{\bf x}}
\newcommand{\yvarl}{{\bf y}}

\newcommand{\Pxy}{P_{x,y}} 
\newcommand{\NDetti}{k_3(\mtl,\mzl,\mtl)}
\newcommand{\tHmus}{\mu^2}
\newcommand{\NDstnt}{k_2(\mtl,0,\mtl)}
\newcommand{\NDstzn}{k_2(\mtl,\mzl,0)}
\newcommand{\NDstzns}{k^2_2(\mtl,\mzl,0)}
\newcommand{\NDstzt}{k_2(\mzl,0,\mtl)}
\newcommand{\NDttzt}{k_3(\mtl,\mzl,\mtl)}
\newcommand{\NDttzts}{k^2_3(\mtl,\mzl,\mtl)}
%\newcommand{\rtz}{r_{tz}}
\newcommand{\rtzs}{r^2_{tz}}
\newcommand{\st}{s_{t}}
\newcommand{\mzt}{M^2_{{\sss{Z}}t}}
